An Algebraic Foundation for Knowledge Graph Construction (Extended Version)

Although they exist since more than ten years already, have attracted diverse implementations, and have been used successfully in a significant number of applications, declarative mapping languages for constructing knowledge graphs from heterogeneous types of data sources still lack a solid formal foundation. This makes it impossible to introduce implementation and optimization techniques that are provably correct and, in fact, has led to discrepancies between different implementations. Moreover, it precludes studying fundamental properties of different languages (e.g., expressive power). To address this gap, this paper introduces a language-agnostic algebra for capturing mapping definitions. As further contributions, we show that the popular mapping language RML can be translated into our algebra (by which we also provide a formal definition of the semantics of RML) and we prove several algebraic rewriting rules that can be used to optimize mapping plans based on our algebra.

==> algorithms/srcopparam_algo.tex <==

\begin{algorithm}[htbp]
    \SetArgSty{textnormal}
    \DontPrintSemicolon
	\caption{\textsc{SrcOpParams} - creates
		%the parameters for a source operator to be created for a given triples map.}
		parameters for a source operator.}
	\label{alg:rml_source_op}
        \KwData{%
            $\triplesMapIRI_\textsf{tm}$ - IRI or blank node of the triples map
	            %for which the source operator is to be created
	            %to create the source operator for \;
	            to create the operator for \;
				\hspace{10mm}
		    $\symRMLGraph$ - an RDF graph (assumed to contain a \emph{normalized} RML description)
        }

        \KwResult{ a tuple $(\dataSource, \queryExpr, \symAttrQueryMap)$
			%to be used as
			of
        parameters for a source operator (as per Definition~\ref{def:source_operator})}

		$u_\textsf{ls} \gets o$, where $o \in \symAllIRIs \cup \symAllBNodes$ such that $(\triplesMapIRI_\textsf{tm},\ttlSmaller{rml:logicalSource},o) \in \symRMLGraph$ \;

		$\dataSource \gets \fctInitSrc{u_\textsf{ls}}$
        \tcp*[r]{Definition~\ref{def:init_data_source}}

		$\queryExpr \gets \lex$, where $o \in \symAllLiterals$ such that $(u_\textsf{ls},\ttlSmaller{rml:iterator},o) \in \symRMLGraph$, with $o = (\lex,\dt)$ \;

		$\symAttrQueryMap \gets \textsc{ExtractQueries}(\triplesMapIRI_\textsf{tm}, \symRMLGraph)$
		\tcp*[r]{Algorithm~\ref{alg:query_extraction}}

		\Return{$(\dataSource, \queryExpr, \symAttrQueryMap)$}
\end{algorithm}

